Enhancing Label Consistency on Document-level Named Entity Recognition

Named entity recognition (NER) is a fundamental part of extracting information from documents in biomedical applications. A notable advantage of NER is its consistency in extracting biomedical entities in a document context. Although existing document NER models show consistent predictions, they still do not meet our expectations. We investigated whether the adjectives and prepositions within an entity cause a low label consistency, which results in inconsistent predictions. In this paper, we present our method, ConNER, which enhances the label dependency of modifiers (e.g., adjectives and prepositions) to achieve higher label agreement. ConNER refines the draft labels of the modifiers to improve the output representations of biomedical entities. The effectiveness of our method is demonstrated on four popular biomedical NER datasets; in particular, its efficacy is proved on two datasets with 7.5-8.6% absolute improvements in the F1 score. We interpret that our ConNER method is effective on datasets that have intrinsically low label consistency. In the qualitative analysis, we demonstrate how our approach makes the NER model generate consistent predictions. Our code and resources are available at https://github.com/dmis-lab/ConNER/.

==> sections/usecase.tex <==
% \section {Use Cases of \ours}

% We introduce two use cases in which \bern~\citep{kim2019neural} was used in the field of biomedical information extraction.
% For these cases, \ours~can directly replace \bern~with faster and more accurate inference.

% \textbf{Biomedical knowledge graph construction}
% Biomedical literature contains considerable amount of expert knowledge.
% Constructing biomedical knowledge graphs from the biomedical literature can help researchers navigate this information more easily.
% Biomedical entities extracted by~\ours~can be used as essential components~(e.g., nodes in the graphs) when building biomedical knowledge graphs.
% For example, \cite{xu2020building} use~\bern~to automatically extract biomedical entities from 29 million PubMed abstracts and build a PubMed knowledge graph, utilizing the extracted entities as nodes.


% \textbf{Biomedical entity-based search engine}
% As biomedical documents are rich in domain-specific terminology, extracting named entities can enhance search engines to find documents related to the entities in queries.
% Vapur~\citep{koksal2020vapur}, which is a search engine for finding protein compounds in COVID-19 literature, pre-process a document into a set of triples~(\textit{Entity1}, \textit{Relation}, \textit{Entity2}).
% They adopt~\bern~to recognize and normalize the named entities in a document so that relevant documents that contain the same concepts can be retrieved.
% For example, if "IL1B" is given as a query, Vapur retrieves documents that not only contain "IL1B", but also "Interleukin1b", since they are normalized to the same concept~(EntrezGene:3553) by \bern.


% \vspace{-0.5cm}
